Autodata: An agentic data scientist to create high quality synthetic data

We introduce Autodata, a general method that enables AI agents to act as data scientists who build high quality training and evaluation data. We show how to train (meta-optimize) such a data scientist agent, so that it learns to create even stronger data. We describe the overall formulation, and a specific practical implementation, Agentic Self-Instruct. We conduct experiments on computer science research tasks, legal reasoning tasks and reasoning with mathematical objects, where we obtain improved results compared to classical synthetic dataset creation methods. Further, meta-optimizing the data scientist agent itself delivers an even larger performance uplift. Agentic data creation provides a way to convert increased inference compute into higher quality model training. Overall, we believe this direction has the potential to change the way we build AI data.

==> main_agent_prompt.tex <==
\begin{table}[p]
\centering
\caption{Instructions for the main agent in the agentic self-instruct setup used in our mathematical reasoning experiments.}
\label{tab:main_instructions}
\begin{adjustbox}{max totalsize={0.98\linewidth}{0.88\textheight},center}
\begin{tcolorbox}[
  colback=gray!10,
  colframe=gray!40,
  boxrule=0.4pt,
  arc=0.8mm,
  left=1mm,right=1mm,top=1mm,bottom=1mm,
  width=0.98\linewidth
]
\begin{minipage}{0.965\linewidth}
\begin{Verbatim}[fontsize=\footnotesize,breaklines=true,breakanywhere=true]
# Main Agent

Generate a question-answer pair that satisfies the success criteria. You will see specific task and domain about the question in the user prompt.

## Success Criteria -- MANDATORY, NO EXCEPTIONS

These are hard pass/fail gates. A question is accepted ONLY when BOTH conditions hold simultaneously. There is zero tolerance for ambiguity.

With `--runs-per-solver 4`:

1. **Weak solver MUST FAIL:** Out of 4 attempts, the weak solver may produce AT MOST 1 correct answer. (<=1 correct out of 4). If the weak solver gets 2 or more correct, the question is REJECTED.
2. **Strong solver MUST SUCCEED:** Out of 4 attempts, the strong solver may produce AT MOST 1 wrong answer. (>=3 correct out of 4). If the strong solver gets 2 or more wrong, the question is REJECTED.

**Do not approximate, do not round, do not use "majority" heuristics.** Count the exact numbers from the evaluation report and compare against the thresholds above.

## Question and Answer Format Requirements

- **Atomic questions only.** Each question must ask exactly ONE thing. No multi-part questions, no "and also", no sub-questions. If you find yourself using semicolons or conjunctions to join separate asks, split them -- then pick the single best one.
- **One-sentence answers.** The correct answer must be expressible in a single sentence. This ensures the verifier can reliably compare predictions against the reference. Avoid long derivations, lists, or multi-paragraph answers.
- **Verifiable answers.** Avoid answers that are bare integers (too guessable) or real numbers subject to precision errors. Prefer exact symbolic forms, named entities, or short phrases that admit unambiguous equivalence checking.

## Tools

- `challenger` subagent -- generates and refines questions (use via task tool)
- `evaluate.py` CLI tool -- the ONLY way to test questions against solvers

### evaluate.py Usage

```bash
pixi run python3 .opencode/tools/evaluate.py \
    --problem "Your problem statement here" \
    --expected-answer "The expected answer" \
    --solvers weak,strong \
    --runs-per-solver 4 \
    --output-dir ./eval_attempts \
    --config .opencode/tools/api_config.json
```

You must use at least 15 minutes timeout on the bash tool. Dependencies are managed by pixi (see `pixi.toml`). For additional packages: `pixi add --pypi <package>`.

Arguments:
- `--problem`: The problem statement to evaluate (required)
- `--expected-answer`: The expected correct answer (required)
- `--solvers`: Comma-separated solver names -- e.g. `weak`, `strong`, or `weak,strong` (default: `weak,strong`)
- `--runs-per-solver`: Number of parallel runs per solver. **Use 4 for both weak and strong.**
- `--output-dir`: Base directory for results (default: `./eval_attempts`)
- `--config`: Path to API config JSON (default: `.opencode/tools/api_config.json`)
\end{Verbatim}
\end{minipage}
\end{tcolorbox}
\end{adjustbox}
\end{table}
\begin{adjustbox}{max totalsize={0.98\linewidth}{0.88\textheight},center}
\begin{tcolorbox}[
  colback=gray!10,
  colframe=gray!40,
  boxrule=0.4pt,
  arc=0.8mm,
  left=1mm,right=1mm,top=1mm,bottom=1mm,
  width=0.98\linewidth
]
\begin{minipage}{0.965\linewidth}
\begin{Verbatim}[fontsize=\footnotesize,breaklines=true,breakanywhere=true]
The tool spawns solver LLMs in parallel, verifies each answer against the expected answer using a verifier LLM, and writes:
- Per-solver attempt files (`weak_solver_run0.txt`, etc.) with full reasoning
- `difficulty_report.json` with structured results
- A markdown summary printed to stdout

## Workflow

### Step 1: Generate Candidate Questions in Parallel

Spawn **multiple challenger subagents in parallel** (3-5 at once) with varied angles, difficulty strategies, or phrasings for the given domain. Each challenger should produce a distinct candidate question-answer pair.

### Step 2: Screen Candidates (Your Judgment)

Read all challenger outputs. Use your own reasoning to assess which candidates are most likely to satisfy the success criteria -- i.e., hard enough to trip the weak solver but clear enough for the strong solver. Discard obviously weak candidates without wasting evaluation budget.

### Step 3: Evaluate with evaluate.py

Run `evaluate.py` **only on the promising candidates** you selected in Step 2. This is expensive -- do not evaluate every idea. Use `--runs-per-solver 4` and `--solvers weak,strong`.

**You MUST use `evaluate.py` for ALL solver testing. Do NOT spawn solver or verifier subagents manually. Do NOT try to simulate solver behavior yourself.**

### Step 4: Analyze Evaluation Results

After each evaluation run:
1. Read the markdown summary printed to stdout. Check the exact counts: weak correct <=1 AND strong correct >=3.
2. If criteria are NOT met, read the per-solver attempt files from `./eval_attempts/run_*/` to understand WHY:
   - If weak solver is succeeding: identify what makes the question too easy and tell the challenger specifically what to change.
   - If strong solver is failing: identify where it goes wrong and tell the challenger how to make the question more tractable for a careful reasoner.
3. Feed this analysis back to a challenger subagent with precise instructions on what to adjust.

### Step 5: Iterate Until Criteria Met

Repeat Steps 1–4. Do not stop until the success criteria are met with exact counts.

### Step 6: Save Final Output

When criteria are met, write the final question and answer to `./question_answer.json`:

```json
{
  "question": "...",
  "answer": "..."
}
```

## Rules

- Do not stop until the success criteria (<=1 weak correct, >=3 strong correct out of 4) are met
- Use `evaluate.py` for ALL solver testing -- no manual solver/verifier subagents
- Every question must be atomic (single question) with a one-sentence answer
- Analyze solver attempt files after every evaluation to give targeted feedback to challengers
- Ensure answer formatting instructions are included in every challenger request so the reference answer is unambiguous
\end{Verbatim}
\end{minipage}
\end{tcolorbox}
\end{adjustbox}
\end{table}

